On biological flow networks: Antagonism between hydrodynamic and metabolic stimuli as driver of topological transitions

A plethora of computational models have been developed in recent decades to account for the morphogenesis of complex biological fluid networks, such as capillary beds. Contemporary adaptation models are based on optimization schemes where networks react and adapt toward given flow patterns. Doing so, a system reduces dissipation and network volume, thereby altering its final form. Yet, recent numeric studies on network morphogenesis, incorporating uptake of metabolites by the embedding tissue, have indicated the conventional approach to be insufficient. Here, we systematically study a hybrid-model which combines the network adaptation schemes intended to generate space-filling perfusion as well as optimal filtration of metabolites. As a result, we find hydrodynamic stimuli (wall-shear stress) and filtration based stimuli (uptake of metabolites) to be antagonistic as hydrodynamically optimized systems have suboptimal uptake qualities and vice versa. We show that a switch between different optimization regimes is typically accompanied with a complex transition between topologically redundant meshes and spanning trees. Depending on the metabolite demand and uptake capabilities of the adaptating networks, we are further able to demonstrate the existence of nullity re-entrant behavior and the development of compromised phenotypes such as dangling non-perfused vessels and bottlenecks.

==> Sections/theory.tex <==
\section{Theory}\label{sec:theory}
 In this section we give a brief reminder on the theoretical framework of fluid advection and metabolite transport Kirchhoff networks. For readers already familiar with these concepts we propose to skip forward to section \ref{sec:results}.
\subsection{Approximating capillary beds as Kirchhoff networks}\label{sec:basic_circuit}
\input{./Sections/theory_transport_model_kirchhoff}
\subsection{Metabolite transport in lumped network models}\label{sec:metabolite uptake}
\input{./Sections/theory_transport_model_meigel}

\subsection{Multi-target driven radius optimization}\label{sec:optimization}
\input{./Sections/theory_optimization}

\subsection{Measuring topological network redundancy and metabolite filtration}
\label{sec:orderparameters}
\input{./Sections/theory_order_parameter}
